Pictures Of MIDI: Controlled Music Generation via Graphical Prompts for Image-Based Diffusion Inpainting

Recent years have witnessed significant progress in generative models for music, featuring diverse architectures that balance output quality, diversity, speed, and user control. This study explores a user-friendly graphical interface enabling the drawing of masked regions for inpainting by an Hourglass Diffusion Transformer (HDiT) model trained on MIDI piano roll images. To enhance note generation in specified areas, masked regions can be "repainted" with extra noise. The non-latent HDiTs linear scaling with pixel count allows efficient generation in pixel space, providing intuitive and interpretable controls such as masking throughout the network and removing the need to operate in compressed latent spaces such as those provided by pretrained autoencoders. We demonstrate that, in addition to inpainting of melodies, accompaniment, and continuations, the use of repainting can help increase note density yielding musical structures closely matching user specifications such as rising, falling, or diverging melody and/or accompaniment, even when these lie outside the typical training data distribution. We achieve performance on par with prior results while operating at longer context windows, with no autoencoder, and can enable complex geometries for inpainting masks, increasing the options for machine-assisted composers to control the generated music.

==> figs/hourglass_arch.tex <==
\newcommand{\hditblock}[6]{
    \begin{scope}[rotate=-90]
        \node[standard node={white},minimum height=2.5mm,transform shape,minimum width=#5] at #2 (hditblocklayer1#1) {};

        \foreach \x in {2,...,#4} {
            \pgfmathtruncatemacro{\xlast}{\x - 1}
            \node[standard node={white},minimum height=2.5mm,above=2.5mm of hditblocklayer\xlast#1,minimum width=#5,transform shape] (hditblocklayer\x#1) {};
            \draw[standard arrow] (hditblocklayer\xlast#1) -- (hditblocklayer\x#1);
        }
        
        \begin{scope}[on background layer]
            \node[
                standard node={green},
                label={[align=center]above:{#3}},
                fit=(hditblocklayer1#1) (hditblocklayer1#1) (hditblocklayer#4#1) (hditblocklayer#4#1),
                minimum width=0,
                minimum height=0,
            ] (hditblock#1) {};
        \end{scope}
    \end{scope}
}
\newcommand{\tokenmergename}{2$\times$2 Pixelunshuffle\\Merge + Proj.}
\newcommand{\tokensplitname}{Proj.+ 2$\times$2\\Pixelshuffle Split}

\begin{tikzpicture}
    \begin{scope}[rotate=-90]
        \node[standard node={gray},minimum width=64mm,transform shape] (inputimage) {Image Input};
        \node[standard node={blue},minimum width=61mm,trapezium,trapezium stretches body,above=of inputimage,transform shape] (patching) {Patching ($p \times p$)\\+ Embedding};
        \draw[standard arrow] (inputimage) -- (patching);
    \end{scope}
    
    \hditblock{1}{($(patching) + (0,11mm)$)}{Neighborhood\\\modelname{} Blocks}{2}{47mm}{1}
    \draw[standard arrow] (patching) -- (hditblocklayer11);
    
    \begin{scope}[rotate=-90]
        \node[standard node={blue},minimum width=50mm,trapezium,trapezium stretches body,above=6mm of hditblock1.east,transform shape] (tokenmerge1) {\tokenmergename};
        \draw[standard arrow] (hditblocklayer21) -- (tokenmerge1);
    \end{scope}
    
    \hditblock{2}{($(tokenmerge1) + (0,11mm)$)}{Neighborhood\\\modelname{} Blocks}{2}{36mm}{2}
    \draw[standard arrow] (tokenmerge1) -- (hditblocklayer12);
    
    \begin{scope}[rotate=-90]
        \node[standard node={blue},minimum width=39mm,trapezium,trapezium stretches body,above=6mm of hditblock2.east,transform shape] (tokenmerge2) {\tokenmergename};
        \draw[standard arrow] (hditblocklayer22) -- (tokenmerge2);
    \end{scope}

    


    
    \hditblock{3}{($(tokenmerge2) + (0,11mm)$)}{Global\\\modelname{} Blocks}{5}{\tikzstyleminimumwidth}{3}
    \draw[standard arrow] (tokenmerge2) -- (hditblocklayer13);


    
    \begin{scope}[rotate=-90]
        \node[standard node={blue},minimum width=39mm,trapezium,trapezium left angle=120,trapezium right angle=120,trapezium stretches body,above=of hditblock3.east,transform shape] (tokensplit1) {\tokensplitname};
        \draw[standard arrow] (hditblocklayer53) -- (tokensplit1);
    \end{scope}
    \node[standard node circle={white}, right=of tokensplit1.north] (lerp1) {\small lerp};
    \draw[standard arrow] (tokensplit1) -- (lerp1);
    \draw[standard arrow] (hditblocklayer22.north) -- ++(4mm,0) |- ++(0,-22.5mm) -| (lerp1);
    
    \hditblock{4}{($(lerp1) + (0,10mm)$)}{Neighborhood\\\modelname{} Blocks}{2}{36mm}{2}
    \draw[standard arrow] (lerp1) -- (hditblocklayer14);
    
    \begin{scope}[rotate=-90]
        \node[standard node={blue},minimum width=50mm,trapezium,trapezium left angle=120,trapezium right angle=120,trapezium stretches body,above=of hditblock4.east,transform shape] (tokensplit2) {\tokensplitname};
        \draw[standard arrow] (hditblocklayer24) -- (tokensplit2);
    \end{scope}
    \node[standard node circle={white}, right=of tokensplit2.north] (lerp2) {\small lerp};
    \draw[standard arrow] (tokensplit2) -- (lerp2);
    \draw[standard arrow] (hditblocklayer21.north) -- ++(4mm,0) |- ++(0,-28mm) -| (lerp2);
    
    \hditblock{5}{($(lerp2) + (0,10mm)$)}{Neighborhood\\\modelname{} Blocks}{2}{47mm}{1}
    \draw[standard arrow] (lerp2) -- (hditblocklayer15);
    
    \begin{scope}[rotate=-90]
        \node[standard node={blue},above=of hditblock5.east,minimum width=50mm,transform shape] (outnorm) {RMSNorm};
        \draw[standard arrow] (hditblocklayer25) -- (outnorm);
        \node[standard node={blue},minimum width=61mm,trapezium,trapezium left angle=120,trapezium right angle=120,trapezium stretches body,above=of outnorm,transform shape] (tokensplit3) {Proj. + $p \times p$\\Pixelshuffle};
        \draw[standard arrow] (outnorm) -- (tokensplit3);
        \node[standard node={gray},above=of tokensplit3,minimum width=64mm,transform shape] (outputimage) {Image Output};
        \draw[standard arrow] (tokensplit3) -- (outputimage);
    \end{scope}
\end{tikzpicture}

